On Sampling, Anonymization, and Differential Privacy: Or, k-Anonymization Meets Differential Privacy

This paper aims at answering the following two questions in privacy-preserving data analysis and publishing: What formal privacy guarantee (if any) does $k$-anonymization provide? How to benefit from the adversary's uncertainty about the data? We have found that random sampling provides a connection that helps answer these two questions, as sampling can create uncertainty. The main result of the paper is that $k$-anonymization, when done "safely", and when preceded with a random sampling step, satisfies $(\epsilon,\delta)$-differential privacy with reasonable parameters. This result illustrates that "hiding in a crowd of $k$" indeed offers some privacy guarantees. This result also suggests an alternative approach to output perturbation for satisfying differential privacy: namely, adding a random sampling step in the beginning and pruning results that are too sensitive to change of a single tuple. Regarding the second question, we provide both positive and negative results. On the positive side, we show that adding a random-sampling pre-processing step to a differentially-private algorithm can greatly amplify the level of privacy protection. Hence, when given a dataset resulted from sampling, one can utilize a much large privacy budget. On the negative side, any privacy notion that takes advantage of the adversary's uncertainty likely does not compose. We discuss what these results imply in practice.

==> background.tex <==
%!TEX root = ./Privacy.tex

%In this paper we deal with publishing relational microdata, that is, the input dataset consists of tuples, each of which corresponds to one individual.  Other interesting types of data exist, such as social network data and network trace data, but they are beyond the scope of this paper and provide for some interesting future work.  

We would like to answer the questions ``whether differential privacy is needed for microdata publishing?'', and ``what exactly is wrong with the $k$-anonymity notion''.  We approach this by examining real world privacy incidents and identifying what aspects are common between them. We show that these disclosures all fall into a general class that we call positive membership disclosures.  In such an disclosure, when given the published dataset, an adversary can find a tuple $t$ and assert with high confidence that $t$ in the original dataset.

\subsection{Privacy Incidents}\label{sec:reiden:incidents}

As privacy is a social concept, any formalization of privacy must be based on what the society perceives as privacy breaches.  In this section, we analyze the well-publicized privacy incidents in data publishing in recent years, and identify the common features of what the society considered to be privacy breaches.

An early and well publicized privacy incident is from the supposedly anonymized medical visit data made available by the Group Insurance Commission (GIC)~\cite{Swe02a}.  While the obvious personal identifiers are removed, the published data included zip code, date of birth, and gender, which are sufficient to uniquely identify a significant fraction of the population.  Sweeney~\cite{Swe02a} showed that by correlating this data with the publicly available Voter Registration List for Cambridge Massachusetts, medical visits about many individuals can be easily identified, including those of William Weld, a former governor of Massachusetts.  We note that even without access to the public voter registration list, the same privacy breaches can occur.  Many individuals' birthdate, gender and zip code are public information.
 %For any individual that is in the dataset, there would be many people who know these attributes of the individual and can who can subsequently re-identify the individual's data. T
This is especially the case with the advent of social media, including Facebook, where users share seemingly innocuous personal information to the public.

Another well-known privacy incident came from publishing web search logs.  In 2006, AOL released three months of search logs involving 650,000 users. The only privacy protection technique used is replacing user ids with random numbers. This proved to be a failure. Two New York Time journalists \cite{BZ06} were able to re-identify Thelma Arnold, a 62 year old women living in Lilburn, Ga. from the published search logs.  Ms. Arnold's search log includes her last name and location names near where she lived.  The reporters were able to cross-reference this information with phonebook entries.  After the New York Time article is published, the data was immediately retracted by AOL.  Later a class action lawsuit was filed against AOL. This scandal led to the resignation of AOL's CTO and the dismissal of two employees.

%The journalists were able to tie Ms. Arnold to specific search queries she made. This included searching for her last name, her friend's ailments, and location names near where she lived.  While some of these queries seem innocuous by themselves, their combination proved to pose a serious privacy risk. 


%\todo{What happened afterwards?  Data retracted. People fired.  Lawsuit?} %The information used to identify Ms. Arnold comes from Ms. Arnold's search queries such as last name or geological key words.

In 2009, Netflix released a dataset containing the movie rating data from 500,000 users as part of a one-million dollar challenge to the data mining research community for developing effective algorithms for predicting users' movie preferences based on their viewing history and ratings.  %This micro-data dataset is high dimensional and sparse.
While the data was anonymized in order to protect users' privacy,  Narayanan and Schmatikov~\cite{NS08} showed that an adversary who has some knowledge about a subscriber's movie viewing experience can easily identify the subscriber's record if it is present in the dataset.  For example, \cite{NS08} shows that, from the profiles of 50 IMDB users, at least 2 of them also appear in the Netflix dataset.
%Narayanan and Shmatikov~\cite{NS09} later extended their work to de-anonymizing social network data.  They developed a re-identification algorithm identify individuals in social networks using only the structure of the network.
 %that can correlate nodes in two anonymized social networks using only network structure information.
%Because we focus on relational data in this paper, we learn lessons mostly from the Netflix attack.

Another privacy incident targeted the Genome-Wide Association Studies (GWAS).  These studies normally compare the DNA of two groups of participants: people with the disease (cases) and similar people without (controls). Each person's DNA mutations (single-nucleotide polymorphisms, or SNPs) at indicative locations are read, and the data is then analyzed.  Traditionally, researchers publish aggregate frequencies of SNPs for participants in the two groups.  In 2008, Homer et al.~\cite{HSR+08} proposed attacks that could tell with high confidence whether an individual is in the case group, assuming that the individual's DNA is known.  The attack works even if the group includes hundreds of individuals.  Because of the privacy concerns from such attacks, a number of institutions, including the US National Institute of Health (NIH) and the Wellcome Trust in London all decided to restrict access to data from GWAS.  
%Wang et al.'s work \cite{WLW+09} improved the attack techniques to reduce the number of required SNPs.  
Such attacks need access to the victim's DNA data and publicly available genomic database to establish the likely SNP frequencies in the general population.

%\todo{Give a little more details about the following attacks.  Include the genomics privacy.} There have been several well-publicized privacy breach incidents in recent years. Examples include the identification of the medical record of the governor of Massachusetts from the GIC data~\cite{Swe02a}; the identification of the search history of an AOL user from the AOL query log data~\cite{BZ06}; and the linking of some Netflix subscribers from the Netflix Prize dataset to users of the IMDB database~\cite{NS08}.

In this paper, we use these four privacy incidents, namely, GIC, AOL, Netflix, and GWAS, as our guiding examples of what the society consider as privacy breaches.

\subsection{Lessons from Privacy Incidents}

From these incidents, we learn the following lessons:
\begin{itemize}
 \item
 \emph{Re-identification matters.}
In the GIC, AOL, and Netflix incidents, one is able to correctly identify \emph{one individual}'s record from supposedly anonymous data.  This fact alone is sufficient for the society to agree that privacy is breached.  It doesn't matter whether an adversary is able to learn additional sensitive information about one individual.
%In other words, re-identification is what the society views as the most clear form of privacy violation.

 \item
 \emph{Positive assertion of membership matters.}
In the GWAS example, only aggregate information is published and there is no individual record to point to.  However, so long as the adversary can positively assert that one individual's data is in the input dataset based on the output, this is a privacy breach.  
%Later our analysis will show that the boundary between re-identification and positive assertion of membership is actually quite blurred.
%In the case of GWAS privacy concerns, the published data is aggregated statistics, hence re-identification takes the form of reaching a high confidence conclusion that a particular individual's data is in the original dataset.

 \item
 \emph{Must protect everyone.}
In several attacks, only a single individual is re-identified; however, that is sufficient to cause widespread privacy concerns and serious consequences (e.g., the AOL case).  This suggests that privacy protection must apply to \emph{every individual}.  A method that on average offers good protection, but may compromise some individual's privacy is not acceptable.

 \item
\emph{No separation of Quasi-Identifier and Sensitive Attributes.}
Much of database privacy research assumes the division of all attributes into quasi-identifiers (QIDs) and sensitive attributes (SA), where the adversary is assumed to know the QIDs, but not SAs.  This separation, however, is very hard to obtain in practice.  No such separation exists in the cases of AOL, Netflix, or GWAS.  Even though only some attributes are used in the GIC incident, it is difficult to assume that they are the only QIDs.  Other attributes in the GIC data includes visit date, diagnosis, etc.  There may well exist an adversary who knows this information about some individuals, and if with this knowledge these individuals' record can be re-identified, it is still a serious privacy breach.  The same difficulty is true for publishing any kind of census, medical, or transactional data.  When publishing anonymized microdata, one has to defend against all kinds of adversaries, some know one set of attributes, and others know a different set.  An attribute about one individual may be known by some adversaries, and unknown (and thus should be considered sensitive) for other adversaries.  It seems that the only reasonable assumption one can make is the following:

\begin{quote}\textbf{[Complete Individual Knowledge Assumption]}
For every individual, there may exist an adversary who knows \emph{all attributes} of that individual.
\end{quote}

 \item
\emph{The adversary relies on one individual's information for re-identification of that individual.}
We note that in the privacy incidents, when re-identifying one individual, the adversary uses only that individual's specific information, and does not rely on the specific information of any other tuples.

We stress that complete individual knowledge assumption is weaker than assuming that there is an adversary who knows \emph{all attributes of all individuals} in the dataset.
\end{itemize}

\subsection{Positive Membership Disclosure}

The above analysis suggest that a privacy breach is a re-identification and positive assertion of membership for some tuple $t$ that may be known by the adversary.  Intuitively, re-identifying a tuple $t$ means that an adversary is able to point to some feature of the output dataset, and conclude that this feature reflects that $t$ is in the input dataset.  However, it is difficult to formalize what constitutes a ``feature''.  In Section~\ref{sec:kanon}, we show that $k$-anonymity fails to prevent re-identification because it implicitly requires the adversary to point to a single tuple for re-identification, when in fact multiple tuples may be related to one input tuple $t$.  Hence we must allow the adversary to point to a larger granularity of the output than a single tuple.  As there is no natural granularity to stop, even when an adversary points to the output as a whole, and say that this output occurs because it contains an input tuple $t$, this should still be considered a re-identification.  Along this line of reasoning, we give the following informal description of re-identification.

%\begin{definition}[Re-Identification]\label{def:reiden}
\begin{quote}\label{def:reiden}
\textbf{Re-Identification:} Given an input dataset $D$, we say that the output $S=\AA(D)$ is subject to a re-identification attack, when there exists a tuple $t\in D$ such that an adversary can say with confidence: the fact that $S$ is output indicates that $t$ is in the input dataset.
\end{quote}
%\end{definition}

Note that whether re-identification occurs or not is not just a property of the output $S=\AA(D)$.  In order to say that $S$ indicates $t$ is in the input dataset, one must consider the behavior of the algorithm $\AA$ on datasets that do not include $t$.  In particular, if even when $t$ is not in the input dataset, the output $S$ is just likely to occur, it is difficult to say that $S$ indicates that $t$ is in the input.

The above informal characterization of re-identification is very similar to positive membership disclosure, which we formalize below.

\begin{definition}\label{def:PMD}
\textbf{[Positive Membership Disclosure (PMD)]:} We say that an algorithm $\AA$ has $\gamma$-positive membership disclosure under a class $\mathbb{D}$  of prior beliefs on output $S\in \mathsf{range}(\AA)$ when there exists a distribution $\DD \in \mathbb{D}$ and a tuple $t$ such that when $\mathbf{D}\leftarrow \DD$ (i.e., $\mathbf{D}$ is drawn according to the distribution \DD), we have
$$\frac{\Pr[t\in \mathbf{D} |S]}{\Pr[t\in \mathbf{D}]} > \gamma \mbox{ or } \frac{\Pr[t\not\in \mathbf{D} |S]}{\Pr[t\not\in \mathbf{D}]} < \frac{1}{\gamma}$$
\end{definition}
We define $0/0$ to be $1$, and $p/0$ to be $\infty$ when $p>0$.
The intuition of a positive membership disclosure is that when an adversary's prior belief (i.e., background knowledge) is that the input dataset is drawn from the distribution $\DD$, then after observing $S$ as the output, the adversary's belief that $t$ is in the input dataset increases by a factor greater than $\gamma$, or the adversary's belief that $t$ is not in the input dataset decreases by a factor greater than $\gamma$.

The above definition is parameterized on the set $\mathbb{D}$, each member of which is a probability distribution of the input datasets, representing a possible prior belief about the input datasets. 

Observe that in order to avoid a positive membership disclosure, it must be
$$\frac{\Pr[t\in \mathbf{D} |S]}{\Pr[t\in \mathbf{D}]} \leq \gamma \mbox{ and } \frac{\Pr[t\not\in \mathbf{D} |S]}{\Pr[t\not\in \mathbf{D}]} \geq \frac{1}{\gamma},$$
which implies that
$$\Pr[t\in \mathbf{D} |S] \leq \min(\gamma \Pr[t\in \mathbf{D}], 1- \frac{1}{\gamma}\Pr[t\not\in \mathbf{D}]).$$
For example, suppose that $\Pr[t\in \mathbf{D}]=0.85$, and $\gamma=1.2$, then $\Pr[t\in \mathbf{D} |S] \leq \min(1,0.875)=0.875$.  The $0.875$ bound is because $\Pr[t\not\in \mathbf{D} |S]$ is lower-bounded by $(1-0.85)/1.2=0.125$.

The following lemma provides a sufficient condition for preventing the positive membership disclosure condition to occur.

\begin{lemma} \label{lemma:noPMD}
For any \DD, if $\frac{\Pr[S | t\in \mathbf{D}]}{\Pr[ S | t\not\in \mathbf{D}]} \leq \gamma$, then the positive membership disclosure condition will not occur.
\end{lemma}
\begin{proof}
Let $\frac{\Pr[S | t\in \mathbf{D}]}{\Pr[ S | t\not\in \mathbf{D}]}=r$, then
$$
\begin{array}{ll}
 \frac{\Pr[t\in \mathbf{D} |S]}{\Pr[t\in \mathbf{D}]}  & = \frac{ \Pr[S | t\in \mathbf{D}] } {\Pr[S]}
 \\
 & = \frac{ \Pr[S | t\in \mathbf{D}] } { \Pr[S | t\in \mathbf{D}] \Pr[t \in \mathbf{D}] + \Pr[S | t\not\in \mathbf{D}] \Pr[t \not\in \mathbf{D}]}
\\
  & = \frac{r  \Pr[S | t\not\in \mathbf{D}] } { r\Pr[S | t\not\in \mathbf{D}] \Pr[t \in \mathbf{D}] + \Pr[S | t\not\in \mathbf{D}] \Pr[t \not\in \mathbf{D}]}
\\
 & = \frac{r  } { r \Pr[t \in \mathbf{D}] + \Pr[t \not\in \mathbf{D}]}
\\
 & \leq \max(r,1) \leq \gamma
\end{array}
$$
At the same time, we also have
$$
\begin{array}{ll}
\frac{\Pr[t\not\in \mathbf{D} |S]}{\Pr[t\not\in \mathbf{D}])}  & = \frac{ \Pr[S | t\not\in \mathbf{D}] } {\Pr[S]}
\\
 & = \frac{ \Pr[S | t\not\in \mathbf{D}] } { \Pr[S | t\in \mathbf{D}] \Pr[t \in \mathbf{D}] + \Pr[S | t\not\in \mathbf{D}] \Pr[t \not\in \mathbf{D}]}
\\
 & =  \frac{ \Pr[S | t\not\in \mathbf{D}] } { r\Pr[S | t\not\in \mathbf{D}] \Pr[t \in \mathbf{D}] + \Pr[S | t\not\in \mathbf{D}] \Pr[t \not\in \mathbf{D}]}
\\
 & =  \frac{1 } { r \Pr[t \in \mathbf{D}] + \Pr[t \not\in \mathbf{D}]}
\\
 & \geq \min(1,\frac{1}{r}) \geq \frac{1}{\gamma}
\end{array}
$$
\end{proof}

Definition~\ref{def:PMD} is parameterized by  $\DD$.  Unfortunately, no positive membership disclosure under arbitrary prior beliefs is impossible to achieve unless the algorithm is trivial, as shown by the following lemma.

\begin{lemma}\label{lemma:noPMD}
If an algorithm \AA has \textbf{no} $\gamma$-positive membership disclosure under $\mathbb{D}_U$, where includes all distributions, then for any pair of datasets $(D_1,D_2)$ such that there exists a tuple $t$ that appears in one of $D_1,D_2$ but not the other, it must be
$\forall S \frac{ \Pr[\AA(D_1)=S] }{\Pr[\AA(D_2)=S] } \leq \gamma$.
\end{lemma}
\begin{proof}
\comment{
First, the ``if'' direction.  For any distribution \DD, we show that $\frac{\Pr[S | t\in D]}{\Pr[ S | t\not\in D]} \leq e^{\epsilon}$, we guarantees no positive membership disclosure by Lemma~\ref{lemma:nomembership}.  Let $p=\min_{D} \Pr[S|D]$, then $\max_{D} \Pr[S|D] \leq e^{\epsilon}p$.
$$
%\begin{array}{ll}
 \frac{\Pr[S | t\in D ]}{\Pr[S | t\not\in D]}
 & = \frac{\frac{ \sum_{D_1:t \in D_1}  \Pr[\AA(D_1) = S] \Pr[D_1]}{\sum_{D_1:t \in D_1}\Pr[D_1]}}
     {\frac{ \sum_{D_2:t\not\in D_2} \Pr[\AA(D_2)=S] \Pr[D_2]}{\sum_{D_2:t\not\in D_2}\Pr[D_2]}}
 \\
 & \leq \frac{\frac{ \sum_{D_1:t \in D_1}  e^{\epsilon}p \Pr[D_1]}{\sum_{D_1:t \in D_1}\Pr[D_1]}}
     {\frac{ \sum_{D_2:t\not\in D_2} p \Pr[D_2]}{\sum_{D_2:t\not\in D_2}\Pr[D_2]}}
 \\
 & = e^{\epsilon}
\end{array}
$$
}
Assume that there exists $D_1$ and $D_2$ and $S$ such that
 $$\frac{ \Pr[A(D_1)=S] }{\Pr[A(D_2)=S] } = r > \gamma,$$
then let $t$ be a tuple that exists in one of $D_1,D_2$ but not the other.  There are two cases.

Case one: $t$ is in $D_1$, but not $D_2$, then choose $p$ to be any number in $\left(0,\frac{r-\gamma}{\gamma(r-1)}\right)$, and use the distribution $\DD=\{\tuple{D_1:p}, \tuple{D_2:1-p}\}$, which means $D_1$ occurs with probability $p$, and $D_2$ with $1-p$, we have
$$
\begin{array}{ll}
 \frac{\Pr[t\in D |S]}{\Pr[t\in D]}  & = \frac{ r } {r p + 1-p} > \frac{r}{\frac{r(r-\gamma)+\gamma(r-1)-(r-\gamma)}{\gamma(r-1)}} = \gamma
\end{array}
$$
Case two: $t$ is in $D_2$, but not $D_1$, choose  $p$ to be any number in $\left(0,\frac{\gamma-1}{r-1}\right)$, and use the distribution $\DD=\{\tuple{D_1:p}, \tuple{D_2:1-p}\}$, we have
$$
\begin{array}{ll}
 \frac{\Pr[t\not\in D |S]}{\Pr[t\not\in D]}  = \frac{1}{rp+1-p} < \frac{1}{\frac{r(\gamma-1)+(r-1)-(\gamma-1)}{r-1}} = \frac{1}{\gamma}
\end{array}
$$
\end{proof}

We stress that the above necessary condition for no positive membership disclosure under arbitrary prior beliefs is extremely strong, as it requires the outputs of $\AA$ on \emph{any two} datasets are close, no matter how different these two datasets are.  In the next section we will show that $\epsilon$-Differential Privacy protects against positive membership disclosure under certain limited kinds of prior beliefs. 
